Handover Experiments with UAVs: Software Radio Tools and Experimental Research Platform

Mobility management is the key feature of cellular networks. When integrating unmanned aerial vehicles (UAVs) into cellular networks, their cell association needs to be carefully managed for coexistence with other cellular users. UAVs move in three dimensions and may traverse several cells on their flight path, and so may be subject to several handovers. In order to enable research on mobility management with UAV users, this paper describes the design, implementation, and testing methodology for handover experiments with aerial users. We leverage software-defined radios (SDRs) and implement a series of tools for preparing the experiment in the laboratory and for taking it outdoors for field testing. We use solely commercial off-the-shelf hardware, open-source software, and an experimental license to enable reproducible and scalable experiments. Our initial outdoor results with two SDR base stations connected to an open-source software core network, implementing the 4G long-term evolution protocol, and one low altitude UAV user equipment demonstrate the handover process.

==> include/research.tex <==
%The envisioned platform needs to be able to serve the advanced wireless and UAS research and development (R\&D) communities. We therefore conducted an extensive literature survey and identified several current research topics in Table I, where initial research results have been reported based on theoretical analyses, simulations and, to a limited extent, experimentation. We also conducted a broad user survey among global researchers. Out of 71 responses, 51 are from professors, 6 are from graduate students, and the rest includes people from industry, Idaho National Labs, NASA, and the German Aerospace Center.
%Survey outcomes show that having (1) access to training tutorials/videos, (2) the  ability to reserve the testbed, (3) the  ability to access the platform through multiple means, and (4) 

As part of our AERPAW project, we conducted a survey among researchers and professors. It was determined that full remote access to SDRs is a critical feature.  
There was significant interest to use SDRs at cell towers and at the UAS. 
Having access to mmWave SDRs and 5G NR mobile phones carried by the UAS were also highly demanded. 
For UAS applications, search and rescue, detection and tracking, and the use of UAVs as hot spot BSs received the highest interest.
Additional experimentation possibilities were suggested by the survey takers. 
These include mobile VR/AR, %the use of wireless communications for control/guidance of multi-agent networks, e.g. in micro-grid scenarios, 
%energy endurance of aerial platforms,
propagation measurements, %wireless energy transfer,  %from UAS to distant sensors,
multi-connectivity with UAVs, high resolution imaging/surveying, UWB,  %localization/communication,
computational and energy efficient protocols, %dynamic/adaptive bandwidth allocation, %to support UAS search and rescue operations, design of 
multi-band and multi-function microwave/mm-wave circuits, and extended UAS command and control using cellular and wireless local area networks \cite{aerpaw_vtc}. 

A flexible and highly efficient experimental research platform is needed to support research on these use cases. 
Moreover, such platform should allow \textit{reproducibility} of experiments, \textit{usability} for quick on-boarding of new users, \textit{interoperability} with new hardware and software, \textit{programmability} of radios and networks, \textit{open access} to spur innovation, and \textit{diversity} of experiments and users. 
%While custom UAS radio designs will , 
Modern software radio technology, high-density computing, and flexible or plug-and-play RF front ends facilitate using programmable radio systems for development, prototyping, of new wireless technology and services. 

%\begin{table}[t!]
%\caption{Aerial wireless research challenges.} %and example recent literature.} %(in \textcolor{red}{red} by AERPAW team).}
%\small 
%\begin{tabular}{|m{2cm}|m{5.9cm}|}
%\hline
%\textbf{%Wireless 
%Challenge } & \textbf{Description and representative publication} 
%& \textbf{AERPAW Contact / Potential Users}
%& \textbf{Papers} 
%\\ \hline 
%mmWave communications & Aerial communication/propagation at different mmWave frequencies, link distances, speeds, and environmental conditions~\cite{rupasinghe2017non}.%,xiao2016enabling}.
%$%~\cite{rupasinghe2017non,UAVhoverOpt_Globecom2016,kong2017autonomous,xiao2016enabling}%,hur_mmwave}. %Experiments with emerging mmWave phased array platforms in highly-mobile 3D aerial environments. 
%$%& Rappaport, Matolak, Guvenc, Love / FIU, NCSU, GSU, Purdue Ruhr Univ. 
%$%& \textcolor{red}{\cite{rupasinghe2017non,UAVhoverOpt_Globecom2016}} \cite{kong2017autonomous,xiao2016enabling,hur_mmwave}   
%\\ \hline
%3D antenna design and aerial MIMO & Single/multiple antenna structures to support full 3D coverage and UAS maneuvers%An initial approach for such designs is via full-wave electromagnetic field solvers followed by AERPAW validation
%%& Adams, Floyd, Hughes, Love / Purdue, GSU, USC, MSU, DLR, UNT  
%~\cite{chen2018impact}.%,mozaffari2018communications}.
%%~\cite{chen2018impact,mozaffari2018communications}
%\\ \hline
%Trajectory optimization & 
%Operating UAS in BVLOS scenarios require 
%Seamless, reliable, autonomous UAS connectivity to a fixed wireless/cellular network on ground through trajectory design~\cite{john2017cooperative}.%,wu2018joint}. 
%%~\cite{bulut2018trajectory,john2017cooperative,Moin_RWS,Moin_Aerospace,wu2018joint,zeng2017energy}
%%Considering UAS connectivity constraints and other mission requirements, AERPAW will support autonomous path planning and trajectory optimization experiments in a controlled environment.  
%%& Dutta, Guvenc / VT, VCU, OSU, Purdue, INL, UPC, UNT, PSS, NUS 
%%& \textcolor{red}{\cite{bulut2018trajectory,john2017cooperative,Moin_RWS,Moin_Aerospace}} \cite{wu2018joint,zeng2017energy}   
%\\ \hline
%UAS-BS placement optimization &  
%%While there are numerous research papers in the literature on 3D placement of UAS-BSs and relays to serve terrestrial users, realistic propagation conditions and antenna radiation/placement effects are typically ignored. AERPAW will allow to 
%Placement optimization %experiments 
%with UAS and aerial balloons serving as relays/BSs under real propagation conditions~\cite{UABSforPSC_VTmag2016}.%,8038869}. 
%%s~\cite{UABSforPSC_VTmag2016,UAVregretLearning_Globecom2016,kumbhar2018exploiting,7486987,8038869,bor2018environment,7762053}
%%& Guvenc / VT, VCU, Purdue, UBC, INL, MSU, Wiser, ANRA, TTech, PSS 
%%& \textcolor{red}{\cite{UABSforPSC_VTmag2016,UAVregretLearning_Globecom2016,kumbhar2018exploiting}}\cite{7486987,8038869,bor2018environment,7762053}   
%\\ \hline
%Channel measurements and modeling %%measurements/modeling  
%& %Depending on location, UAS enable communication from a nearly continuous range of heights, and a large variety of horizontal positions as well, hence conventional terrestrial channel models are insufficient. AERPAW will enable 
%Propagation measurements and practical channel models for various 3D UAS locations, environments, frequencies~\cite{Wahab_Aerospace}.%%,matolak2017air2}. 
%%~\cite{khawaja2016uwb,khawaja2017uav,Wahab_Aerospace,matolak2017air,sun2017air,matolak2017air2,sun2017air2,al2018modeling,cai2017low,amorim2017radio,goddemeier2015investigation,greenberg2017channel}
%%& Matolak, Rappaport, Guvenc  / OSU, UBC, USC, INL, DLR, UNT, Wiser, PSS, NCSU, Univ. Sydney  
%%& \textcolor{red}{\cite{khawaja2016uwb,khawaja2017uav,Wahab_Aerospace,matolak2017air,sun2017air,matolak2017air2,sun2017air2}} \cite{al2018modeling,cai2017low,amorim2017radio,goddemeier2015investigation,greenberg2017channel}   
%\\ \hline
%wireless security  & Data/GPS signal jamming, side channel attacks, and physical layer security with UAS~\cite{menouar2017uav}.%,wang2017improving}. 
%%~\cite{DronesSmartCities_IWCMC2016,UAVsmartcities_CommMag2016,park2017persistent,hagerman2016security,rodday2016exploring,wang2017improving}
%%will be some of the wireless security experiments that will be supported by AERPAW.   
%%& Marojevic, Dai / INL, FIU, NCSU, UBC, VT, Ruhr Univ., MSU, USF, TTech 
%%& \textcolor{red}{\cite{DronesSmartCities_IWCMC2016,UAVsmartcities_CommMag2016} }  \cite{yoon2017security,park2017persistent,hagerman2016security,rodday2016exploring,wang2017improving}  
%\\ \hline
%Wireless localization/tracking %%with UAS  
%& Localize, identify, track wireless devices/users at UAS based on RF signals~\cite{koohifar2018autonomous}.%,qi2016search}. 
%%~\cite{MultiUAVtracking_CommLett2015,koohifar2018autonomous,acuna2017localization,van2018autonomous,wang2017guideloc,qi2016search,chen2016real,ho2015krypto}
%%, with applications to search and rescue of victims and surveillance of intruders.   
%%& Sichitiu, Guvenc / OSU, Purdue, NCSU, MSU,  DLR, UNT, Wiser, UNCC, WildTrack, IIT Delhi
%%& \textcolor{red}{\cite{MultiUAVtracking_CommLett2015,koohifar2018autonomous,acuna2017localization}} \cite{van2018autonomous,wang2017guideloc,al2018modeling,qi2016search,chen2016real,ho2015krypto}  
%\\ \hline
%Multi-hop and ad hoc UAS networks & Range extension and intra/inter-swarm UAS communications for improved autonomy and reliability~\cite{chen2018multiple}.%,kakar2018uav}. 
%%~\cite{Fouda_VTC,Moin_Aerospace,zhang2018trajectory,chen2018multiple,li2018placement,challita2017network,liu2018transceiver}
%%& Sichitiu, Guvenc, Love / VCU, Purdue,  INL, UNT, UNCC, NED, NASA Glenn 
%%& \textcolor{red}{\cite{Fouda_VTC,Moin_Aerospace}} \cite{zhang2018trajectory,chen2018multiple,li2018placement,challita2017network,liu2018transceiver,marcum_netcode}   
%\\ \hline
%Spectrum sharing %with UAS  
%& Spectrum activity monitoring and sharing with agile/mobile UAS and balloons~\cite{zhang2017spectrum}.%yuksel2016pervasive, 
%%~\cite{yuksel2016pervasive,merwaday2015uav,athukoralage2016regret,chen2011collaborative,lyu2017spectrum,zhang2017spectrum}
%%& Sichitiu, Wang / OSU,  USC, MSU, UNT, FIU, Covenant Univ., UPF, NASA Glenn 
%%& \textcolor{red}{\cite{kakar2017waveform,yuksel2016pervasive,merwaday2015uav,athukoralage2016regret}} \cite{chen2011collaborative,lyu2017spectrum,zhang2017spectrum,kim_milcom,marcum_milcom}
%\\ \hline
%Waveform design &  Experiments with new waveforms %(FBMC, OTFS, etc.) 
%to combat unique multipath/Doppler characteristics of UAS~\cite{kakar2017waveform}. %jamal2017fbmc,
%+%~\cite{jamal2017fbmc,jamal2018dual,jamal2016multicarrier,sahin2014survey,ma20165g,sacchi2018filter,wu2005performance,abualhaol2010performance}
% communications %necessitate the design, testing, evaluation of new waveforms, such as dual-polarized filter-bank multi-carrier and orthogonal time frequency space modulations, which will be enabled by AERPAW.  
%& Matolak, Marojevic, Love / INL, MSU, Purdue, USF, UNCC, DLR, WildTrack, 
%&  \textcolor{red}{\cite{jamal2017fbmc,jamal2018dual,jamal2016multicarrier,sahin2014survey,kakar2017waveform}} \cite{ma20165g,sacchi2018filter,wu2005performance,abualhaol2010performance}   
%\\ \hline
%UAS Detection \& tracking & RF and radar based unauthorized  / malicious / non-cooperating UAS %may cause extensive damage to public, government, and military settings. AERPAW will support both RF-based and radar-based 
%detection, classification, and tracking~\cite{koohifar2018autonomous}.%,azari2018key}. 
%~\cite{Ezuma_RWS,Martins_Aerospace,guvenc2018detection,guvencc2017detection,MultiUAVtracking_CommLett2015,koohifar2018autonomous,azari2018key,ding2018amateur,solomitckii2018technologies}
%&Guvenc, Matolak / MSU, INL, DLR, Wiser, WildTrack, NCSU 
%& \textcolor{red}{\cite{Ezuma_RWS,Martins_Aerospace,guvenc2018detection,guvencc2017detection,MultiUAVtracking_CommLett2015,koohifar2018autonomous}}  \cite{azari2018key,ding2018amateur,solomitckii2018technologies} 
%\\ \hline
%SDN, Cloud, edge comput. & Edge processing/caching at UAS, SDN for mesh UAS networking~\cite{zavesky2018systems}.%,chen2017caching}. 
%%~\cite{kakar2018uav,zavesky2018systems,7932923,7744808,narang2017cyber,chen2017caching,moradi2018skycore}
%%& Dutta, Lin, Marojevic / Purdue, NCSU, GSU, VCU, FIU 
%%& \textcolor{red}{\cite{kakar2018uav}} \cite{zavesky2018systems,7932923,7744808,narang2017cyber,chen2017caching,moradi2018skycore}   
%\\ \hline
%IoT design and applications & Using UAS to monitor agriculture, environmental, infrastructure IoT sensors~\cite{motlagh2017uav}.%,polo2015design}. 
%%~\cite{Vageesh_RWS,motlagh2017uav,yoo2016flying,polo2015design,costa2012use,bacco2014uavs}
%%& Dutta / OSU, Purdue, UBC, Wiser, NCSU, UNCC, IIT Delhi
%%& \textcolor{red}{\cite{Vageesh_RWS}} \cite{motlagh2017uav,yoo2016flying,polo2015design,costa2012use,bacco2014uavs} 
%\\ \hline
%Command and control %for UAS NAS integration 
%& Communications, command, networking, autonomy protocols for multi-UAS flights in national airspace~\cite{koohifar2018autonomous}.%,kakar2017waveform}. 
%%~\cite{MultiUAVtracking_CommLett2015,koohifar2018autonomous,consiglio2012concepts,munoz2014family,fern2012uas,weibel2005integrated}
%%& Hayes, Snyder / ASSURE, NCSU, USC, UNT, ANRA, PSS, NASA Glenn 
%%& \textcolor{red}{\cite{MultiUAVtracking_CommLett2015,koohifar2018autonomous}} \cite{consiglio2012concepts,munoz2014family,fern2012uas,weibel2005integrated}  
%\\ \hline
%UAS integration into cellular & UAS experiments with underlying 4G/5G cellular infrastructure and vehicular wireless infrastructure~\cite{amorim2017radio}.%,john2017cooperative,zhou2015multi}. 
%%~\cite{menouar2017uav,bulut2018trajectory,john2017cooperative,Moin_RWS,Moin_Aerospace,kovacs2017interference,amorim2017radio,zhou2015multi}
%%& Marojevic, Guvenc / OSU, GSU, VT, InterDigital, NCSU, NASA Glenn  
%%& \textcolor{red}{\cite{menouar2017uav,bulut2018trajectory,john2017cooperative,Moin_RWS,Moin_Aerospace}} \cite{kovacs2017interference,amorim2017radio,zhou2015multi}   
%\\ \hline
%\end{tabular}\label{tab:T_FI}\vspace{-.45cm}%\vspace{-0.15cm}
%\end{table}


%The AERPAW team will prioritize the experimentation options in the platform, and will look into possibility of gradually introducing new functionality in future years to match user demands.
